Eliminating Backdoors in Neural Code Models for Secure Code Understanding

Neural code models (NCMs) have been widely used to address various code understanding tasks, such as defect detection. However, numerous recent studies reveal that such models are vulnerable to backdoor attacks. Backdoored NCMs function normally on normal/clean code snippets, but exhibit adversary-expected behavior on poisoned code snippets injected with the adversary-crafted trigger. It poses a significant security threat. Therefore, there is an urgent need for effective techniques to detect and eliminate backdoors stealthily implanted in NCMs. To address this issue, in this paper, we innovatively propose a backdoor elimination technique for secure code understanding, called EliBadCode. EliBadCode eliminates backdoors in NCMs by inverting/reverse-engineering and unlearning backdoor triggers. Specifically, EliBadCode first filters the model vocabulary for trigger tokens based on the naming conventions of specific programming languages to reduce the trigger search space and cost. Then, EliBadCode introduces a sample-specific trigger position identification method, which can reduce the interference of non-backdoor (adversarial) perturbations for subsequent trigger inversion, thereby producing effective inverted backdoor triggers efficiently. Backdoor triggers can be viewed as backdoor (adversarial) perturbations. Subsequently, EliBadCode employs a Greedy Coordinate Gradient algorithm to optimize the inverted trigger and designs a trigger anchoring method to purify the inverted trigger. Finally, EliBadCode eliminates backdoors through model unlearning. We evaluate the effectiveness of EliBadCode in eliminating backdoors implanted in multiple NCMs used for three safety-critical code understanding tasks. The results demonstrate that EliBadCode can effectively eliminate backdoors while having minimal adverse effects on the normal functionality of the model.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> algorithms/code_search_trigger_inversion.tex <==
\begin{algorithm}[htbp]
    \caption{GCG-based Trigger Inversion on Code Search Task}
    \footnotesize
    \label{alg:trigger_inversion_on_code_search}
    %\vspace{2.5pt}
    %\hspace{-15.5mm}
    \raggedright
    \begin{tabular}{rllll}
        %\toprule
        \hline
        \textsc{Input}: & $X^m$ & \; & selected masked samples & \\
        & $V$ & \; & trigger vocabulary & \\
        & $V_g$ & \; & target vocabulary & \\
        & $f_{\theta^*}$ & \; & backdoored NCM & \\
        & $\epsilon$ & \; & times of iterations & \\
        & $k$ & \; & number of candidate substitutes & \\
        & $r$ & \; & times of repeat \\
        & $\beta$ & \; & threshold for trigger anchoring & \\
        
        \textsc{Output}: & $t^*$ & \; & anchored trigger & \\
        & $g^*$ & \; & inverted target & \\
        %\bottomrule
        \hline
    \end{tabular}
    \begin{algorithmic}[1]
        \Function{TriggerInversion}{$S^m$, $Q$}
            \State $t, g \gets $ randomly initialize a trigger with $n$ tokens and a target with $m$ tokens from $V$ and $V_g$, respectively
    
            \State $\bm{e}_{S^m}, \bm{e}_{Q} \gets$ produce embeddings of code snippets in $S^m$ and embeddings of query in $Q$ using $f_{\theta^*}$
            
            \For{$z=0, z<\epsilon$, z++}
                \State $o_t, o_g \gets$ generate the one-hot representation of $t$ and the one-hot representation of $g$
                
                \State $\bm{e}_t,\bm{e}_g \gets$ produce $o_t$'s embeddings and $o_g$'s embeddings using $f_{\theta^*}$
    
                \State $\bm{e}'_{S^m} \gets \bm{e}_{S^m} \oplus \bm{e}_t$
                \State $\bm{e}'_{Q} \gets \bm{e}_{Q} \oplus \bm{e}_g$
        
                \State $G \gets \nabla o_t\mathcal{L}(f_{\theta^*}(\bm{e}'_{S^m}), \bm{e}'_{Q})$
                \State $G_g \gets \nabla o_g\mathcal{L}(f_{\theta^*}(\bm{e}'_{S^m}), \bm{e}'_{Q})$
    
                \State $\mathcal{T}, \mathcal{T}_g \gets$ select substitutes for each trigger token based on top-$k$ gradients of $o_t$ in $G$ and $o_g$ in $G_g$, respectively
        
                \State $t^C \gets \emptyset$ \hfill\Comment{\textcolor{gray}{store candidate substitute triggers}}
                \State $g^C \gets \emptyset$ \hfill\Comment{\textcolor{gray}{store candidate substitute targets}}
                \For{$j = 1, j < r, j++$}
                    \State $t^{j},g^{j} \gets t, g$
                    \State $i, u \gets$ randomly select a position to be replaced in $t^{j}$ and $g^{j}$, respectively
                    
                    \State $\mathcal{T}_i, \mathcal{T}_{g_u} \gets $ get all candidate substitutes for $i$-th token of $t^j$ and $u$-th token of $g^j$, respectively
                
                    \State $t_{i}^{j}, g_{u}^{j} \gets$ randomly select a substitute from $\mathcal{T}_i$ and $\mathcal{T}_{g_u}$, respectively
        
                    \State $t^{j}, g^{j} \gets$ replace the $i$-th token of $t^{j}$ with $t_{i}^{j}$  and the $u$-th token of $g^{j}$ with $g_{u}^{j}$, respectively
                    
                    \State $t^C \gets$ $t^C \cup t^{j}$
                    \State $g^C \gets$ $g^C \cup g^{j}$
                \EndFor
                \State $x \gets t^C \times g^C$ 
                \hfill\Comment{\textcolor{gray}{all possible ordered pairs of $t^C$ and $g^C$}}
                \State $t \gets x_{j}.t, g \gets x_{j}.g$, where $j = \mathop{\arg\min}_j\mathcal{L}(f_{\theta^*}(S^m \oplus x_{j}.t),Q \oplus x_{j}.g), j \in [1, r^2]$
                \hfill\Comment{\textcolor{gray}{compute best substitution}}
                
            \EndFor
            \State \Return $t$, $g$
        \EndFunction
        \\
        \Function{TriggerAnchoring}{$S^m$, $Q$, $t$, $g$}
            \State $t^* \gets \emptyset$
            \State $l \gets \mathcal{L}(f_{\theta^*}(S^m \oplus t), Q \oplus g)$
            \For{each token $t_i$ \textbf{in} $t$}

                \State $l_i \gets \mathcal{L}(f_{\theta^*}(S^m \oplus (t \setminus t_i)), Q \oplus g)$
                
                \If{$|l-l_i| > \beta$}
                    \State $t^* \gets t^* \cup t_i$
                \EndIf
            \EndFor
            \State \Return $t^*$
        \EndFunction
        \\
        
        \State $<S^m, Q> \gets$ get masked code snippets and queries in $X^m$
        \State $t$, $g^* \gets $ \Call{TriggerInversion}{$S^m$, $Q$}

        \State $t^* \gets$ \Call{TriggerAnchoring}{$S^m$, $Q$, $t$, $g^*$}
        \State \Return $t^*$, $g^*$
    \end{algorithmic}
\end{algorithm}


==> tables/ablation_study.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    % \footnotesize
    %\tabcolsep=3pt
    %\renewcommand{\arraystretch}{1.1} 
    \caption{Ablation study. TA: Trigger Anchoring;}
    % \vspace{-2mm}
    \label{tab:ablation_study}
    \begin{tabular}{lccc}
        \toprule
        
        Method & ACC & ASR & Epoch \\
    
        \midrule

         w/o phase (a) & 63.73\% & 100\% & -  \\
         
         w/o phase (b) & 62.57\% & 0.24\% & 52 \\


        w/o TA & 60.98\% & 0.08\% & 25 \\

        \ours{} & 62.57\% & 0.24\% & 25 \\

        \bottomrule
    \end{tabular}
    \vspace{-2mm}
\end{table}


==> tables/adaptive_attacks.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \tabcolsep=2.5pt
    % \footnotesize
    %\renewcommand{\arraystretch}{1.2} 
    \caption{Effectiveness of \ours{} on adaptive attack.}
    \label{tab:adaptive_attacks}
    \begin{tabular}{ccccccc}
        \toprule
        
        \multirow{2}{*}{Trigger size} & \multicolumn{2}{c}{Defect detetion} & \multicolumn{2}{c}{Clone detecion} & \multicolumn{2}{c}{Code search} \\

        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        
        & ACC & ASR & F1 & ASR & MRR & ANR \\
    
        \hline

        5 & 62.74\% & 0.24\% & 96.14\% & 6.34\% & 0.82 & 25.52 \\
        7 & 62.97\% & 2.07\% & 96.34\% & 7.57\% & 0.82 & 24.35 \\
        10 & 62.91\% & 4.84\% & 96.26\% & 9.16\% & 0.82 & 22.47 \\

        
        \bottomrule
    \end{tabular}
    %\vspace{-4mm}
\end{table}

==> tables/combine_results_on_adaptive_attack_and_LLM.tex <==
\begin{table}[!t]
    \centering
    % \hspace{-4mm}
    \scriptsize
    \tabcolsep=1.5pt
    % \footnotesize
    \begin{minipage}[c]{0.4\textwidth}
        \renewcommand{\arraystretch}{1.2} 
        \caption{Effectiveness of \ours{} on adaptive attack.}
        \label{tab:adaptive_attacks}
        \begin{tabular}{ccccccc}
            \toprule
            
            \multirow{2}{*}{Trigger size} & \multicolumn{2}{c}{Defect detetion} & \multicolumn{2}{c}{Clone detecion} & \multicolumn{2}{c}{Code search} \\
    
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
            
            & ACC & ASR & F1 & ASR & MRR & ANR \\
        
            \midrule
    
            5 & 62.74\% & 0.24\% & 96.14\% & 6.34\% & 0.82 & 25.52 \\
            7 & 62.97\% & 2.07\% & 96.34\% & 7.57\% & 0.82 & 24.35 \\
            10 & 62.91\% & 4.84\% & 96.26\% & 9.16\% & 0.82 & 22.47 \\
    
            
            \bottomrule
        \end{tabular}
    %\vspace{-4mm}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.55\textwidth}
        \caption{Performance on code LLM. DD: Defect Detection; CD: Clone Detection; CS: Code Search. %large language model.% 
        }
        %\vspace{-2mm}
        \label{tab:effectiveness_on_StarCoder}
        \begin{tabular}{cccccccc}
            \toprule
            
            \multirow{2}{*}{Attack} & \multirow{2}{*}{Task} & \multirow{2}{*}{Metric} & \multicolumn{5}{c}{StarCoder} \\ 
        
            \cmidrule(lr){4-8}
        
            & & & Undefended & ONION & DBS & AttDef & \ours{} \\
    
            \midrule
            
            \multirow{6}{*}{\rotatebox{90}{CodePoisoner}} & \multirow{2}{*}{DD} & ACC & 61.68\% & 59.98\% & 60.71\% & xxx & 60.65\% \\
            
            & & ASR & 96.57\% & xxx & xxx & xxx & 2.87\% \\
            
            \cmidrule{2-8} 
            
            & \multirow{2}{*}{CD} & F1 & 71.91\% & 69.73\% & 70.15\% & xxx & 70.18\% \\
                                 
            & & ASR & 100\% & xxx & xxx\% & xxx & xxx \\
        
            \cmidrule{2-8} 
            
            & \multirow{2}{*}{CS} & MRR & xxx\% & xxx & xxx\% & xxx & xxx\% \\
    
            & & ANR & xxx\% & xxx & xxx\% & xxx & xxx\% \\
            
            \bottomrule
        \end{tabular}
    \end{minipage}
\end{table}

==> tables/combine_table_figure.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[c]{0.45\linewidth}
        
        %\begin{table}[t]
        \footnotesize
        \tabcolsep=1.5pt
        \renewcommand{\arraystretch}{1.1} 
        \captionof{table}{Comparisons of inverted trigger and factual trigger. TA: Trigger Anchoring; DD: Defect Detection; CD: Clone Detection.}
        \label{tab:trigger_accuracy}
        \begin{tabular}{ccccccc}
        \toprule
        
        \multirow{2}{*}{Task} & \multicolumn{2}{c}{DBS} & \multicolumn{2}{c}{w/o TG} & \multicolumn{2}{c}{\ours{}} \\ 
    
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    
        & LD & BLEU & LD & BLEU & LD & BLEU\\
    
        \hline
        
        DD & 19  & 9.27 & 16 & 19.62 & 6 & 29.56 \\

        \hline

        CD & 14  & 8.20 & 14 & 23.30 & 5 & 36.79 \\
        
        \bottomrule
    \end{tabular}
    %\end{table} 
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.46\linewidth}
        %\begin{figure*}[htbp]
        \centering
        \includegraphics[width=\linewidth]{figures/effectiveness_of_different_numbers_of_clean_samples.pdf}
        \caption{Influence of the numbers of clean samples.}
        \label{fig:effectiveness_of_different_numbers_of_clean_samples}
        %\end{figure*}
    \end{minipage}
    \vspace{-4mm}
    %\vspace{-13pt}
\end{figure}


==> tables/effectiveness_on_StarCoder.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \tabcolsep=1.5pt
    \caption{Performance on code large language model. }
    %\vspace{-2mm}
    \label{tab:effectiveness_on_StarCoder}
    % \resizebox{1.0\linewidth}{!}{
    \begin{threeparttable}
    
    \begin{tabular}{cccccccc}
        \toprule
        
        \multirow{2}{*}{Attack} & \multirow{2}{*}{Task} & \multirow{2}{*}{Metric} & \multicolumn{5}{c}{StarCoder} \\ 
    
        \cmidrule(lr){4-8}
    
        & & & Undefended & ONION & DBS & AttDef & \ours{} \\

        \midrule
        
        \multirow{6}{*}{\rotatebox{90}{CodePoisoner}} & \multirow{2}{*}{Defect Detection} & ACC & 61.68\% & 59.98\% & 60.71\% & xxx & 60.65\% \\
        
        & & ASR & 96.57\% & xxx & xxx & xxx & 2.87\% \\
        
        \cmidrule{2-8} 
        
        & \multirow{2}{*}{Clone Detection} & F1 & 71.91\% & 69.73\% & 70.15\% & xxx & 70.18\% \\
                             
        & & ASR & 100\% & xxx & xxx\% & xxx & xxx \\
    
        \cmidrule{2-8} 
        
        & \multirow{2}{*}{Code Search} & MRR & xxx\% & xxx & xxx\% & xxx & xxx\% \\

        & & ANR & xxx\% & xxx & xxx\% & xxx & xxx\% \\
        
        \bottomrule
    \end{tabular}
    \end{threeparttable}
    % }
    % \vspace{-2mm}
\end{table}

==> tables/time_overhead.tex <==
\begin{table*}[t]
    \centering
    \scriptsize
    % \tabcolsep=1.5pt
    %\renewcommand{\arraystretch}{1.2} 
    \caption{Time and cost overhead of \ours{}.}
    %\vspace{-2mm}
    \label{tab:time_overhead}
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cccccccccccc}
        \toprule
        
        \multirow{2}{*}{Attack} & \multirow{2}{*}{Task} & \multirow{2}{*}{Time} & \multicolumn{2}{c}{CodeBERT} & \multicolumn{2}{c}{CodeT5} & \multicolumn{2}{c}{UniXCoder} \\ 
    
        \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    
        & & & DBS & \ours{} & DBS  & \ours{} & DBS & \ours{} \\
    
        %\hline
        \midrule
        
        \multirow{7}{*}{\rotatebox{90}{CodePoisoner}} & \multirow{2}{*}{Defect Detection} & Trigger Inversion & 4m58s & 22m40s & 8m19s & 26m13s & 5m03s & 24m31s  \\

        & & Trigger Unlearning & 0m28s & 0m25s & 1m02s & 1m04s & 0m26s & 0m24s \\
        
        \cmidrule{2-9} 
        
        & \multirow{2}{*}{Clone Detection} & Trigger Inversion & 9m02s & 28m31s & 8m14s & 53m09s & 9m35s & 35m07s \\

        & & Trigger Unlearning & 3m13s & 3m14s & 8m17s & 8m10s & 3m10s & 3m14s \\

        \cmidrule{2-9}
                
        & \multirow{2}{*}{Code Search} & Trigger Inversion & - & 32m25s & - & 26m10s & - & 50m50s \\

        & & Trigger Unlearning & - & 10m58s & - & 30m18s & - & 10m57s \\
        
        \bottomrule
    \end{tabular}
    % }
    % \vspace{-2mm}
\end{table*}

